NL-COMM: Demonstrating Gains of Non-Linear Processing in Open-RAN Ecosystem

Multi-user multiple-input, multiple-output (MU-MIMO) designs can substantially increase wireless systems' achievable throughput and connectivity capabilities. However, existing MU-MIMO deployments typically utilize linear processing techniques that, despite their practical benefits, such as low computational complexity and easy integrability, can leave much of the available throughput and connectivity gains unexploited. They typically require many power-intensive antennas and RF chains to support a smaller number of MIMO streams, even when the transmitted information streams are of low rate. Alternatively, non-linear (NL) processing methods can maximize the capabilities of the MIMO channel. Despite their potential, traditional NL methods are challenged by high computational complexity and processing latency, making them impractical for real-time applications, especially in software-based systems envisioned for emerging Open Radio Access Networks (Open-RAN). Additionally, essential functionalities such as rate adaptation (RA) are currently unavailable for NL systems, limiting their practicality in real-world deployments. In this demo, we present the latest capabilities of our advanced NL processing framework (NL-COMM) in real-time and over-the-air, comparing them side-by-side with conventional linear processing. For the first time, NL-COMM not only meets the practical 5G-NR real-time latency requirements in pure software but also does so within a standard-compliant ecosystem. To achieve this, we significantly extended the NL-COMM algorithmic framework to support the first practical RA for NL processing. The demonstrated gains include enhanced connectivity by supporting four MIMO streams with a single base-station antenna, substantially increased throughput, and the ability to halve the number of base-station antennas without any performance loss to linear approaches.

==> 1_motivation.tex <==
Multi-User Multiple-Input, Multiple-Output (MIMO) and massive-MIMO systems promise a substantial increase in the achievable throughput and connectivity capabilities of wireless communication systems by increasing the wireless link reliability and by enabling the concurrent transmission of multiple information streams over the same frequency. For this reason, and while they already play a significant role in current wireless systems (e.g., 5G), they are expected to play an even more significant role in future communication systems (e.g., 6G) by supporting new use cases for which massive connectivity capabilities and even higher throughout are required (e.g., autonomous driving \cite{5GAmericas2023}, industrial automation \cite{8403588}). While the potential benefits of multi-user MIMO (MU-MIMO) systems are well-documented, the type of signal processing that will unlock the full MU-MIMO potential and will translate it into actual, measurable gains has not yet been finalized. Such kind of processing should not only be capable of translating the MIMO channel capabilities into gains from a theoretical point of view, but it should be practical, power efficient, and able to meet the tight processing latency requirements of current and future wireless developments. It should also account for the  limitations of the current computing platforms, even for systems that are implemented in software, as emerging Open Radio Access Network (Open-RAN) designs envisage \cite{yang_openran_2013,wireless_everything_2020,opsurvey22}. In addition, any new MIMO processing framework should be able to demonstrate clear and indisputable "system-level" benefits when compared to existing ones.

==> 2_openran.tex <==
Open-RAN \cite{yang_openran_2013,wireless_everything_2020,ofcom_open_2022} promises a highly diversified RAN ecosystem, through open disaggregation, interoperability, and the softwarization of digital processing. However, transitioning towards heavily software-based solutions, and particularly implementing 5G-NR MIMO PHY, presents significant design and implementation challenges. This is due to the fact that software-based systems are typically orders of magnitude less computationally efficient compared to dedicated hardware approaches \cite{horowitz20141}. Existing software-based PHY solutions either do not support MU-MIMO \cite{noauthor_srsran_nodate,noauthor_oai_nodate} or deviate substantially from the 5G-NR and Open-RAN standards and principles \cite{yang_bigstation_2013,ding_agora_2020,gong2023hydra}.
%
The absence of practical, comprehensive Open-RAN solutions has compelled world-leading initiatives, such as the UK's Department for Science, Innovation, and Technology (DIST) Future RAN Competition (FRANC), to accelerate the development of high-performance 5G Open RAN solutions by 2025 \cite{ukgov2023open}.
\vspace{-7pt}



==> 3_demo_description.tex <==



\begin{figure}[t]
    \centering
    %\includegraphics[height=2.5cm,width=18.1cm]
    \includegraphics[height=3cm,width=8.1cm]{figures/Fig2.png}
     \vspace{-5pt}
    \caption{The demo setup and the measured over-the-air (OTA) spectral efficiency (SE)}
    \label{fig:sims}
    \vspace{-15pt}
\end{figure}


% Our demo utilizes the first version of our new, purely software-based Open-RAN 5G-NR PHY, which substantially extends and optimizes OpenAirInterface \cite{noauthor_oai_nodate} PHY processing architecture, achieving support for MU-MIMO transmissions and, both, linear and MPNL processing.
% We will demonstrate, for the first time, our highly efficient, MPNL framework, running in real-time and over-the-air, by utilizing a single COTS server and we will compare it against traditional linear processing approaches.
% The attendees will be able to set and change various system parameters, including the placement of the UEs, to validate the substantial throughout and connectivity gains that our MPNL framework can provide. An example case of our demo can be found below \cite{demo2023}


% The attendees will be able to change the placement of the UEs and modify various system parameters (e.g., number of BS antennas, MIMO streams) using a simplified user interface,  to validate MPNL's substantial throughout and connectivity gains. An example case of our demo can be found below \cite{demo2023}

Our demo utilizes our new, purely software-based Open-RAN 5G-NR PHY, which substantially extends and optimizes OpenAirInterface \cite{noauthor_oai_nodate} PHY processing architecture, achieving support for MU-MIMO and, both, linear and MPNL processing. We will demonstrate, for the first time, our highly efficient, MPNL framework, running in real-time and over-the-air, by utilizing a single COTS server and we will compare it against traditional linear processing approaches. The attendees will be able to change the placement of the UEs and, using a simplified user interface, modify various system parameters (e.g., number of BS antennas, MIMO streams), to validate MPNL's substantial throughout and connectivity gains. An example case of our demo can be found below \cite{demo2023}


% The attendees will be able to set and change various system parameters, including the placement of the UEs, to validate the substantial throughout and connectivity gains that our MPNL framework can provide. An example case of our demo can be found below \cite{demo2023}

==> LinearvsMPNL.tex <==
As discussed, the MIMO and massive MIMO (mMIMO) technologies are the ones driving the corresponding connectivity and throughput gains of the latest generation of mobile systems, particularly in the sub-6 GHz frequency range where the multi-path propagation environment allows for large spatial multiplexing gains \cite{goldsmith_capacity_2003,pang_new_2022}. However, depending on the transmission scenario, conventional MIMO deployments with linear processing can leave a lot of the MIMO capacity and connectivity gains unexploited. On the other hand, traditional non-linear processing solutions (e.g., sphere decoders) promise improved throughput and connectivity capabilities, but they are typically of impractical processing complexity and latency when concurrently transmitting a large number of information streams \cite{jalden_complexity_2005,hassibi_sphere-decoding_2005}, and with benefits that have not been validated over-the-air in real-time, 5G-NR and Open-RAN compliant realizations. 


The Massively Parallelizable Non-Linear Processing (MPNL) framework  \cite{nikitopoulos_massively_2022,nikitopoulos2019parallel,nikitopoulos_massively_2019,nikitopoulos_massively_2019-1,husmann_flexcore_2017,nikitopoulos_geosphere_2014,jayawardena_g_multisphere_2020} is the first non-linear transceiver processing scheme that enables the practical concurrent transmission of a large number of streams, with small processing latency. MPNL has the potential to substantially improve the achievable throughput, connectivity, and power consumption of mobile systems, resolving the aforementioned limitations of linear processing. In particular, as shown in the simulation evaluations of Fig.\ref{fig:sims}, over CDL-B \cite{3GPPTR38901} channels,
MPNL can provide the same throughput as linear processing with less than half the number of base station (BS) antennas, resulting in a substantial reduction in the required number of RF chains, saving hundreds of Watts from the base-stations. Moreover, in cases where low-rate, machine-type traffic is involved, MPNL can even support a much larger number of users than base-station antennas, without employing traditional NOMA scheme \cite{saito_noma,nikopour2013sparse,PwrNOMA,SCMAPoC,LDSOFDM,SCMArotate}, enabling practical extreme connectivity. This is in contrast to linear schemes that need a much larger number of base-stations antennas than the number of low-rate transmitted information streams.
%$
% MPNL can support a number of low-rate users that even exceed the number of base station antennas without employing any NOMA scheme. Such capabilities of MPNL can enable extreme connectivity, especially when low-rate machine-type traffic is involved.
%
While initially proposed for MU-MIMO transmissions in the uplink, as we  show here for the first time, MPNL can enable practical non-linear precoding for a large number of streams in the downlink by enabling practical Vector Perturbation 
\cite{VP,MMSEVP,improvedvp,gain15dbvp,FCSE} similar gains as in the uplink, compared to linear precoding.
%
Still, while the potential of MPNL is promising, the implementability of such approaches has not yet been validated in an Open-RAN and 5G-NR compliant setting or by real-time and over-the-air demonstrations, and this is the target of this demo.
\vspace{-4pt}




% \textcolor{red}{briefly explain the gains of MPNL in the downlink (don't site the corresponding conference) compared to linear and gains in throughput and connectivity. Explain how what we show is an extension of the published work. Explain that the results are simulations.}

%Similarly, MPNL applies to the highly complex vector perturbation precoding problem [] in the downlink and can enable practical non-linear precoding for a large number of streams while providing substantial benefits compared to linear processing. In particular, as shown in Fig.\ref{fig:sims}, MPNL can offer the same throughput as linear processing with half the number of base station antennas. In addition,  MPNL can support a number of low-rate users that even exceed the number of base station antennas similar to the uplink. Such evaluations are limited to simulations and have yet to be demonstrated in practice in an Open-RAN-compliant setting.

% \textcolor{red}{briefly explain MPNL compared to other non-linear approaches. the gains of MPNL in the uplink compared to linear (gains in throughput and connectivity). Explain how what we show is an extension of the published work. Explain that the results are simulations.}

%The Massively Parallelizable Non-Linear Processing (MPNL) framework [cite] enables practical near-optimal detection for large MIMO systems in the uplink. In contrast to existing parallelizable detection schemes [], which target the worst-case transmission condition, MPNL can focus the available processing power on the most promising solutions to the MIMO detection problem. MPNL introduces a new mathematical framework to identify these most promising solutions as relative distances before the detection process based only on the transmission channel to achieve this. MPNL can provide substantial throughput and connectivity gains compared to linear processing with similar latency requirements. Additionally, MPNL can offer the same throughput and support the same number of users as linear processing while employing fewer RF chains, substantially reducing power consumption. In particular, as we show by simulation evaluations in Fig.\ref{fig:sims}, MPNL can provide the same throughput as linear processing with less than half the number of base station antennas. Furthermore, MPNL can support a number of low-rate users that even exceed the number of base station antennas without employing any NOMA scheme. However, such gains have not yet been demonstrated in real-time and over-the air, in an  Open-RAN and 5G-NR compliant setting.

==> contributions.tex <==
We demonstrate the first 3GPP and Open-RAN compliant realization of purely software-based PHY, that can support not only linear but also MPNL processing in real-time. This is the first time the substantial gains of MPNL are demonstrated and compared side-by-side to linear approaches, in an Open-RAN and 5G-NR compliant over-the-air setting. The demonstrated MPNL gains include its substantially increased throughput, its ability to halve the number of base-station antennas without any performance loss to linear processing approaches, as well as its ability to support a much larger number of users than base-station antennas.
Moreover, this is the first time that both downlink and uplink MPNL implementation is being realized, proving the implementability of MPNL within a fully-standard compliant setting, by utilizing a single, common commercial-of-the-shelf (COTS) server.
\vspace{-10pt}

